HOI-Ref: Hand-Object Interaction Referral in Egocentric Vision

Large Vision Language Models (VLMs) are now the de facto state-of-the-art for a number of tasks including visual question answering, recognising objects, and spatial referral. In this work, we propose the HOI-Ref task for egocentric images that aims to understand interactions between hands and objects using VLMs. To enable HOI-Ref, we curate the HOI-QA dataset that consists of 3.9M question-answer pairs for training and evaluating VLMs. HOI-QA includes questions relating to locating hands, objects, and critically their interactions (e.g. referring to the object being manipulated by the hand). We train the first VLM for HOI-Ref on this dataset and call it VLM4HOI. Our results demonstrate that VLMs trained for referral on third person images fail to recognise and refer hands and objects in egocentric images. When fine-tuned on our egocentric HOI-QA dataset, performance improves by 27.9% for referring hands and objects, and by 26.7% for referring interactions.

==> sections/dataset.tex <==
To enable hand-object referral and understand the interaction between hands and objects, question-answer pairs with hand-object referral information are required.
Furthermore, to assure that the model is capable of distinguishing across various questions, we follow previous work~\cite{chen2023minigptv2} and use task tags.
In this section, we dive deeper into question-answer pairs and various task tags used to distinguish between them.



\subsubsection{Question-Answer Categories.}

To understand hand-object interaction, we propose a range of question-answer pairs for training.
These pairs can be broadly divided into the following categories:
\begin{enumerate*}[label=(\alph*)]
    \item bounding box in question and hand/object name in answer,
    \item hand/object name in question and bounding box in answer, and
    \item hand/object information (bounding box or name) in question and object/hand information in answer.
\end{enumerate*}
Such question-answer pairs allow the model to understand hand-object interaction and equip it with referral capabilities.
\cref{fig:dataset} summarises the type of questions present in the \dataset dataset.

\subsubsection{Task Tags.}
To ensure that \model is capable of distinguishing between various questions, we adapt the multi-task instruction template proposed in~\cite{chen2023minigptv2}.
As shown in \cref{fig:dataset}, the task tags are added at the beginning of the question.
For \dataset we use \textit{[refer]}, \textit{[grounding]}, \textit{[identify]}, and \textit{[detection]} task tags for question-answers enabling hand-object referral using bounding boxes and \textit{[vqa]} and \textit{[caption]} for question-answer pairs not involving bounding boxes.
\Cref{fig:dataset} shows question-answer pairs from the proposed \dataset.
For example, Question 1 in \cref{fig:dataset} uses the \textit{[identify]} tag to prompt the model to recognise the left hand of the subject.


\subsubsection{Annotation Types.} Finally, to generate the question-answer pairs for the categories mentioned earlier, we use the following annotations:
\begin{enumerate*}[label=(\alph*)]
    \item \textbf{Narrations} to encode the general activity happening in the egocentric image,
    \item \textbf{Object Bounding Boxes} to enhance referral capability of VLMs and to understand hand-object interaction,
    \item \textbf{Hand Bounding Boxes} similar to object bounding boxes, enable referral and improved hand-object interaction understanding,
    \item \textbf{Hand-object contact information} enables referral based on hand-side and object. For example this enables asking questions similar to, \textit{what is in the left hand of the person?} Answering such a question not only requires the model to correctly localise the hand, but also identify the object in that hand.
\end{enumerate*}



\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{images/dataset_v1.2.drawio.pdf}
    \caption{\textbf{\dataset} for training VLMs to understand hand-object interaction.
    We use multiple annotation types to create the question-answer pairs.
    Top half of the figure shows the annotations utilised and the bottom half shows the style of question-answer pairs generated.
    As shown, we convert the segments to bounding boxes to generate various referral questions and utilise contact information to understand interaction between hands and objects.
    Note that manual supervision is not required to create \dataset, making the process scalable.
    }
    \label{fig:dataset}
\end{figure}

\subsubsection{Question-Answer Pairs.}
Here we discuss how various annotation types are converted to question-answer pairs.
Note that \textit{object bounding box} in the following discussion corresponds to the bounding box representation shown in \cref{fig:dataset} and discussed in \cref{subsec:training}.
\begin{enumerate}
    \item \textbf{Narrations} provide us with verb and noun pairs of the action happening in the egocentric image.
    We convert the verb form to its present tense and formulate the sentence as, ``The person \{verb\} the \{noun\}''.
    This sentence is then used as an answer for captioning question.
    For example, \textbf{Question}: \textit{[caption] This is a photo from an ongoing video of hand object interactions. What is happening in the photo?} \textbf{Answer}: \textit{The person opens the tap}. For a visual example, refer to Question 4 in \cref{fig:dataset}.
    \item \textbf{Object Bounding Boxes.}
    We use the object bounding boxes to create the following QA pairs:
    \begin{enumerate*}[label=(\alph*)]
        \item \textbf{Question}: \textit{[refer] Where is the \{object\}?} \textbf{Answer}: \textit{\{Object's bounding box\}};
        \item \textbf{Question}: \textit{[identify] \{Object's bounding box\}}. \textbf{Answer}: \textit{\{Object's name\}};
        \item \textbf{Question}: \textit{[detect] \{Object's name\}}. \textbf{Answer}: \textit{<p>\{Object's name\}</p>} {\{Object's bounding box\}};
        \item \textbf{Question}: \textit{[grounding] This is a photo from an ongoing video of hand object interactions. Describe the ongoing action in this image.} \textbf{Answer}: \textit{The person opens the <p>tap</p> \{tap's bounding box\}}.
    \end{enumerate*}
    For example, Questions 1, 5, 6, and 7 in \cref{fig:dataset}.
    \item \textbf{Hand Object Contact information.} Knowledge about what object the hands are holding is utilised to create the following QA pairs:
    \begin{enumerate*}[label=(\alph*)]
        \item \textbf{Question}: \textit{[vqa] What is the person holding in their \{left/right\} hand?} \textbf{Answer}: \textit{\{Object's name\}};
        \item \textbf{Question}: \textit{[grounding] Describe the ongoing action in this image in detail}. \textbf{Answer}: \textit{The person is working in a kitchen. They are holding a <p>\{object's name\}</p> \{object's bounding box\} in their <p>left hand</p> \{left hand's bounding box\} and a <p>\{object's name\}</p> \{object's bounding box\} in their <p>right hand</p> \{right hand's bounding box\}.}
        \item \textbf{Question}: \textit{[identify] \{left/right hand's bounding box\}}. \textbf{Answer}: \textit{\{Left/right\} hand}.
        \item \textbf{Question}: \textit{[vqa] Is the \{left/right\} hand holding or touching an object?} \textbf{Answer}: \textit{The object in the \{left/right\} hand is a \{object's name\}} OR \textit{\{Left/Right\} hand is not holding anything.}
        \item \textbf{Question}: \textit{[refer] Where is the object being manipulated by the hand?} \textbf{Answer}: \textit{\{object's bounding box in left/right hand\}}.
    \end{enumerate*}
    For example, Questions 2 and 3 in \cref{fig:dataset}.
\end{enumerate}


\begin{table}[!b]
    \centering
    \caption{\textbf{Comparison of referral-based question-answering datasets.} Our \dataset dataset has $52$ times more questions than the current largest third-person dataset and did not require manual efforts to generate it as opposed to Shikra-RD that requires prompting GPT-4}
    \setlength{\tabcolsep}{5pt}
    \begin{adjustbox}{width=1\textwidth}
    \begin{tabular}{@{}lcccc@{}}\toprule
    Dataset & \# QA Pairs & Automatic Generation? & Task Tags? & Egocentric?\\
    \midrule
    Shikra-RD~\cite{chen2023shikra} & $5,922$ & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} \\ 
    Flicker30k~\cite{chen2023minigptv2,7410660} & $2.5$K & \textcolor{green}{\cmark} & \textcolor{red}{\xmark}  & \textcolor{red}{\xmark} \\
    Multi-task Conv.~\cite{chen2023minigptv2} & $60.9$K & \textcolor{green}{\cmark} & \textcolor{green}{\cmark}  & \textcolor{red}{\xmark} \\
    \dataset (ours) & $\mathbf{3.2}$\textbf{M} & \textcolor{green}{\cmark}  & \textcolor{green}{\cmark} & \textcolor{green}{\cmark}\\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:dataset_stats}
\end{table}

\subsubsection{Annotation Sources for Generating Question-Answers.}

Out of various available datasets for egocentric videos~\cite{Damen2022RESCALING,grauman2022ego4d,EgoProceLECCV2022,ragusa_MECCANO_2023,10.1007/978-3-030-01228-1_38,Damen2018EPICKITCHENS}, 
we select EPIC-Kitchens~\cite{Damen2022RESCALING,Damen2018EPICKITCHENS,VISOR2022} and Ego4D~\cite{grauman2022ego4d} as our data source.
This is because EPIC-Kitchens provides crucial hand-object interaction information~\cite{VISOR2022} and Ego4D provides a large quantity of hand and object bounding boxes.
As opposed to egocentric datasets that do not have bounding boxes~\cite{charadesego,EgoProceLECCV2022} or hand-object interaction information~\cite{charadesego,EgoProceLECCV2022,ragusa_MECCANO_2023,10.1007/978-3-030-01228-1_38}.
Out of available annotations in EPIC-Kitchens, we select: 
\begin{enumerate*}[label=(\alph*)]
    \item narrations,
    \item object bounding box annotations from EPIC-Kitchens-55~\cite{Damen2018EPICKITCHENS},
    \item object and hand segments from VISOR~\cite{VISOR2022} (segments are converted to bounding boxes), and
    \item hand object contact information from VISOR~\cite{VISOR2022}.
\end{enumerate*}
From $3,670$ hours of annotations available in Ego4D, we select the subset from forecasting hands and object (FHO) benchmark.
From this subset, we select:
\begin{enumerate*}[label=(\alph*)]
    \item narrations and
    \item bounding boxes for hands and objects.
\end{enumerate*}
As our goal is to enable hand object referral along with hand object interaction understanding, we select the above mentioned subsets from EPIC-Kitchens and Ego4D to create the \dataset dataset.
The rest of the available annotations, for example, audio transcriptions, bounding boxes for faces, and audio action annotations~\cite{EPICSOUNDS2023} are not utilised.

Using the approach mentioned above, we create roughly \textbf{3.2M question-answer pairs} for the \dataset dataset.
Out of 3.2M QA pairs, 1.7M QAs are from EPIC-Kitchen's training set and 1.5M QAs are from Ego4D FHO's training set.
The scale of the proposed \dataset dataset enables training large VLMs like our \model and will fuel future research.
In \Cref{tab:dataset_stats}, we compare \dataset with existing referential-based question-answering datasets. \dataset consists of highest question-answer pairs, is the only dataset for egocentric videos, and does not require prompting a LLM~\cite{chen2023shikra} for its creation resulting in a cleaner set of annotations.
Additional details on diversity of questions and their distribution across task tags are provided in the supplementary.





